Integrating Dark Pattern Taxonomies

The problem of ``Dark Patterns" in user interface/user experience (UI/UX) design has proven a difficult issue to tackle. Malicious and explotitative design has expanded to multiple domains in the past 10 years and which has in turn led to multiple taxonomies attempting to describe them. While these taxonomies holds their own merit, and constitute unique contributions to the literature, their usefulness as separate entities is limited. We believe that in order to make meaningful progress in regulating malicious interface design, we must first form a globally harmonized system (GHS) for the classification and labeling of Dark Patterns. By leaning on network analysis tools and methods, this paper synthesizes existing taxonomies and their elements through as a directed graph. In doing so, the interconnectedness of Dark patterns can be more clearly revealed via community (cluster) detection. Ultimately, we hope that this work can serve as the inspiration for the creation of a glyph-based GHS for the classification of Dark Patterns.

==> 4_GHS.tex <==
\subsection{Impact and Application}

\subsubsection{Heuristic Evaluation}
One potential way to actualize implementing something similar to a GHS for 
Dark Patterns could be to undertake a heuristic evaluation process. Heuristic 
evaluation\cite{Nielson} is a UI/UX evaluation tool prominent in the Human 
Computer Interaction (HCI) space. It began with a set of 
criteria by which to judge the usability of an interface, which were then reduced,
and improved upon over time. The rendered heuristics are then utilized by one 
or more evaluators who make the case that certain heuristics have been violated. 
This process serves to refine the UI at preliminary stages and is a relatively 
low-cost low-effort means to discern exactly what a UI is missing. Because 
heuristic evaluation is less formal and less rigid than other evaluation 
processes, we believe that it suits the unclear, context-based nature of what is considered ``Dark" in certain scenarios. 

Although this work does not have near the rigour or forethought of the GHS for 
hazardous materials, we believe that future work focused on reducing the 
graph and analyzing emerging communities with the intent of forming a new 
heuristic evaluation process for Dark Patterns could serve as a guidepost for 
regulators to create legislation regarding dark patterns in applications and for 
app marketplaces to signal hazards to consumers. Building a glyph-based hazard 
communication system (such as the GHS for hazardous materials) out of an 
existing heuristic evaluation process is as simple as assigning a glyph to 
each heuristic that is violated. A simple proof of concept example can be found 
in figure \ref{fig:heuristic_example}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{./Intermediate_Currency_Warning_Example.png}
    \caption{Violation of the Community 8 inspired Heuristic: ``The value of 
purchasable items is clearly communicated to the purchasing party."}
    \label{fig:heuristic_example}
\end{figure}

